Testing and Learning Quantum Juntas Nearly Optimally

We consider the problem of testing and learning quantum $k$-juntas: $n$-qubit unitary matrices which act non-trivially on just $k$ of the $n$ qubits and as the identity on the rest. As our main algorithmic results, we give (a) a $\widetilde{O}(\sqrt{k})$-query quantum algorithm that can distinguish quantum $k$-juntas from unitary matrices that are "far" from every quantum $k$-junta; and (b) a $O(4^k)$-query algorithm to learn quantum $k$-juntas. We complement our upper bounds for testing quantum $k$-juntas and learning quantum $k$-juntas with near-matching lower bounds of $\Omega(\sqrt{k})$ and $\Omega(\frac{4^k}{k})$, respectively. Our techniques are Fourier-analytic and make use of a notion of influence of qubits on unitaries.

==> sections/intro-final-proj.tex <==
\section{Introduction}
\label{sec:intro}

This paper is motivated by the following natural question: Given query access to a unitary matrix $U$ acting on $n$ qubits, is $U$ of the form $V\otimes I$ for some unitary $V$ acting on $k \ll n$ qubits? If this is the case, we say that the unitary $U$ is a \emph{quantum $k$-junta}. We study this question in the framework of \emph{property testing}, i.e. after defining an appropriate notion of ``distance'' between unitaries, we answer the following question:

\begin{question}[Quantum junta testing] \label{question:qjt}
	Given oracle access to a unitary $U$ and its inverse $U^\dagger$ acting on $n$ qubits and $\eps > 0$, decide with constant probability if $U$ is a $k$-junta or if $\dist(U, V) \geq\eps$ for all quantum $k$-juntas $V$ acting on $n$ qubits. 
\end{question}

\subsection{Prior Work}

We first note that \Cref{question:qjt} captures, as a special case, its classical analog involving classical $k-$juntas. For that, a boolean function $f\isazofunc$ is a $k$-junta if $f(x) = g(x_{i_1}, \ldots, x_{i_k})$ for some $g:\zo^k \to \zo$, and the distance metric used is the normalized Hamming distance. 

\begin{question}[Testing Boolean Juntas]
	Given classical or quantum query access to a function $f\isazofunc$ via a unitary $\calO_f$, decide with constant probability if $f$ is a $k$-junta or if $\dist(f,g)\geq \eps$ for every $k$-junta $g\isazofunc$. 
\end{question} 

This question has been extensively studied over the recent decades. The first result explicitly related to testing juntas was obtained by Parnas, Ron, and Samorodnitsky \cite{Parnas2002}, who gave a \emph{classical} algorithm for testing $1$-juntas with $O(1)$ queries. Soon afterwards, Fischer et al. \cite{Fischer2004} introduced classical algorithms for testing $k$-juntas with $\wt{O}(k^2)$ queries. The query complexity of classically testing juntas was later improved by Blais \cite{Blais2009} who gave a nearly optimal tester which makes $\wt{O}(k)$ queries. Blais's tester is asymptotically optimal up to a logarithmic factor, given the $\Omega(k)$ lower bound for classically testing $k$-juntas by \cite{Chockler2004}.

There has also been a long line of work on testing Boolean juntas via \emph{quantum} algorithms. That is, we are given access to a function $f\isazofunc$ via a unitary $\calO_f$, allowing us to query superpositions of inputs. At\i c\i\ and Servedio \cite{Atici2007} gave an elegant quantum algorithm to test $k$-juntas using $O(k)$ queries.\footnote{At the time \cite{Atici2007} was written, the best classical upper bound on testing juntas was $\wt{O}(k^2)$.} More recently, Ambainis et al. \cite{Ambainis2016} came up with a quantum algorithm to test juntas that makes only $\wt{O}(\sqrt{k})$ queries. This was shown to be essentially optimal by Bun, Kothari, and Thaler~\cite{Bun2017} who proved an $\wt{\Omega}(\sqrt{k})$ lower bound for via a reduction from the image size testing problem.

Returning to \Cref{question:qjt}, Wang \cite{Wang2011} gave a tester for testing whether a unitary operator $U$ is a $k$-junta or is $\eps$-far from a $k$-junta that makes $O(k)$ queries, and their algorithm turns out to be a direct generalization of the tester of At\i c\i\ and Servedio \cite{Atici2007}.\footnote{The result originally obtained by Wang had a worse bound of $O(k\log k)$, but this can be improved to $O(k)$ by following the analysis of \cite{Atici2007} (see Section 5.1.6 of \cite{Montanaro2016}). We also note that their query complexity's dependence on $\eps$ can be improved via a straightforward application of amplitude amplifiaction.} Finally, Montanaro and Osborne \cite{Montanaro2010} had previously studied a different tester for the property of being a ``dictatorship,'' i.e. a $1$-junta, but did not prove correctness. 


\subsection{Our Contributions}

Our main result is a $\wt{O}(\sqrt{k})$-query algorithm for quantum junta testing, which we present in \Cref{sec:testing-ub}. Furthermore, this algorithm is essentially optimal---we prove a near matching lower bound of $\Omega(\sqrt{k})$ in \Cref{sec:lower-bound}. Finally, we provide a $O(\frac{k}{\eps} + \frac{4^k}{\eps^2})$-query algorithm for learning quantum $k-$juntas via membership queries. We also have the following works in progress:
\begin{itemize}
    \item An $\Omega(\sqrt{k})$ lower bound for ``Pauli sampling'' oracles; 
    \item A lower bound for testing if a unitary is a $k$-junta after a change-of-bases.
\end{itemize}

% \subsection{Future Work}

% Things to mention: tolerant testing? distribution free-testing of classical juntas via quantum algorithms?


% {Are channels $k$-juntas or not?}
